Warped Penguins

We present an analysis of the loop-induced magnetic dipole operator in the Randall-Sundrum model of a warped extra dimension with anarchic bulk fermions and an IR brane localized Higgs. These operators are finite at one-loop order and we explicitly calculate the branching ratio for mu to e gamma using the mixed position/momentum space formalism. The particular bound on the anarchic Yukawa and KK scales can depend on the flavor structure of the anarchic matrices. It is possible for a generic model to either be ruled out or unaffected by these bounds without any fine tuning. We quantify how these models realize this surprising behavior. We also review tree-level lepton flavor bounds in these models and show that these are are in mild tension with the penguin bounds from typical models with a 3 TeV Kaluza-Klein scale. Further, we illuminate the nature of the one-loop finiteness of these diagrams and show how to accurately determine the degree of divergence of a 5D loop diagram using both the 5D and KK formalism. This power counting can be obfuscated in the 4D Kaluza-Klein formalism and we explicitly point out subtleties that ensure that the two formalisms agree. Finally, we remark on the existence of a perturbative regime in which these one-loop results give the dominant contribution.

==> diagramsmain.tex <==
\subfloat[$W$ and $H^\pm--W$ loops with two mass insertions. The $W$ loop has an implicit external mass insertion on the $\mu$ line. sf]{\label{fig:main:diagrams:a}
		\begin{tikzpicture}[line width=1.75 pt, scale=1.4]
			% 2MIW
			% \begin{tikzpicture}[line width=1.5 pt, scale=1]
				%
				\draw[fermion] (-1.75,0) -- (-1,0);
				\draw[fermion] (1,0) -- (1.75,0);
				%
				\draw[vector] (-1,0) arc (180:45:1);
				\draw[vector] (45:1) arc (45:0:1); 
				%
				\draw[fermion] (1,0) arc (0:-180:1);
				%
				\draw[vector] (45:1) -- (45:2);
			%
			% MASS INSERTION
			\begin{scope}[rotate=-135]
			\begin{scope}[shift={(1,0)}] % Mass Insertion
				\clip (0,0) circle (.175cm);
				\draw[fermionnoarrow] (-1,1) -- (1,-1);
				\draw[fermionnoarrow] (1,1) -- (-1,-1);
			\end{scope}	
			\end{scope}
			%
			\begin{scope}[rotate=-45]
			\begin{scope}[shift={(1,0)}] % Mass Insertion
				\clip (0,0) circle (.175cm);
				\draw[fermionnoarrow] (-1,1) -- (1,-1);
				\draw[fermionnoarrow] (1,1) -- (-1,-1);
			\end{scope}	
			\end{scope}
			%
			\node at (0,-1.5) {$W$};
			\end{tikzpicture}
			%
			\quad
			%
			% 2MIHW
			\begin{tikzpicture}[line width=1.75 pt, scale=1.4]
				%
				\draw[fermionbar] (-1.75,0) -- (-1,0);
				\draw[fermion] (1,0) -- (1.75,0);
				%
				\draw[scalarnoarrow] (-1,0) arc (180:45:1);
				\draw[vector] (45:1) arc (45:0:1); 
				%
				\draw[fermion] (1,0) arc (0:-180:1);
				%
				\draw[vector] (45:1) -- (45:2);
			%
			% MASS INSERTION
			\begin{scope}[rotate=-135]
			\begin{scope}[shift={(1,0)}] % Mass Insertion
				\clip (0,0) circle (.175cm);
				\draw[fermionnoarrow] (-1,1) -- (1,-1);
				\draw[fermionnoarrow] (1,1) -- (-1,-1);
			\end{scope}	
			\end{scope}
			%
			\begin{scope}[rotate=-45]
			\begin{scope}[shift={(1,0)}] % Mass Insertion
				\clip (0,0) circle (.175cm);
				\draw[fermionnoarrow] (-1,1) -- (1,-1);
				\draw[fermionnoarrow] (1,1) -- (-1,-1);
			\end{scope}	
			\end{scope}
			%
			\node at (0,-1.5) {$H^\pm,W$};
			\end{tikzpicture}
	}               
\qquad 
\subfloat[$W^5$ loop with an implicit mass insertion on the $\mu$ line.]{\label{fig:main:diagrams:b}
			% 0MIW5
			\begin{tikzpicture}[line width=1.75 pt, scale=1.4] 
				%
				\draw[fermion] (-1.75,0) -- (-1,0);
				\draw[fermion] (1,0) -- (1.75,0);
				%
				\draw[vectorscalar] (-1,0) arc (180:45:1);
				\draw[vectorscalar] (45:1) arc (45:0:1); 
				%
				\draw[fermionbar] (1,0) arc (0:-180:1);
				%
				\draw[vector] (45:1) -- (45: 2);
			%%
			\node at (0,-1.5) {$W$};
			\end{tikzpicture}
	}
